Matching on What Matters: A Pseudo-Metric Learning Approach to Matching Estimation in High Dimensions

When pre-processing observational data via matching, we seek to approximate each unit with maximally similar peers that had an alternative treatment status--essentially replicating a randomized block design. However, as one considers a growing number of continuous features, a curse of dimensionality applies making asymptotically valid inference impossible (Abadie and Imbens, 2006). The alternative of ignoring plausibly relevant features is certainly no better, and the resulting trade-off substantially limits the application of matching methods to "wide" datasets. Instead, Li and Fu (2017) recasts the problem of matching in a metric learning framework that maps features to a low-dimensional space that facilitates "closer matches" while still capturing important aspects of unit-level heterogeneity. However, that method lacks key theoretical guarantees and can produce inconsistent estimates in cases of heterogeneous treatment effects. Motivated by straightforward extension of existing results in the matching literature, we present alternative techniques that learn latent matching features through either MLPs or through siamese neural networks trained on a carefully selected loss function. We benchmark the resulting alternative methods in simulations as well as against two experimental data sets--including the canonical NSW worker training program data set--and find superior performance of the neural-net-based methods.

==> blocking.tex <==
The methods described in the previous sections can all be re-purposed for designing maximally efficient and robust experiments. Rather than select matched pairs for analysis in an observational context, we can instead apply our methods in one of three different techniques designed to ensure ideal balance between treated and control samples.

\begin{itemize}
	\item Pair-wise matching: This is a direct extension of our existing methods.
	\item Blocking (stratifying): This does not appear to be an extension of our existing methods. I think blocking should not be viewed as an extension of our method.
	\item Rerandomization: This is not an extension of our existing methods unless we apply the propinquity score.
\end{itemize}

==> ml_matching_methods_intro.tex <==
We propose integrating four separate ML methods into matching estimation. These include two methods for \textit{variable selection} and two for \textit{feature learning}. Variable selection refers to methods which choose a set of matching covariates $X_{select} \subseteq X$, where $X$ is the full set of available covariates. On the other hand, we use ``feature learning" to refer to methods which \textit{construct} a low-dimensional set of features $X_{learn}$. Unlike, $X_{select}$, $X_{learn}$ is not a subset of $X$. Each learned feature $x_{l,i} \in X_{learn}$ is a non-linear combination of the elements in $X$, and it can be assumed that $dim(X_{learn}) < dim(X)$.

These methods are organized as follows:

\begin{itemize}

	\item[1.] \textbf{Variable Selection} 
		
		\begin{itemize}
		
			\item[1a.] \textit{L1 (L1-penalization)}: We estimate two LASSO models, one to predict outcome and one to predict treatment status. We then take either the union or the intersection of the selected features and match on this subset.
						
			\item[2a.] \textit{RRF (Regularized Random Forest)}: We estimate a Regularized Random Forest model following \cite{Deng2012}, one to predict outcome and one to predict treatment status. We then take either the union or the intersection of the selected features and match on this subset.
					
		\end{itemize}
		
	\item[2.] \textbf{Feature Learning}
		
		\begin{itemize}
		
			\item[1b.] \textit{ANN (Artificial Neural Network)}: We estimate two ANN models, one to predict outcome and one to predict treatment status. We then remove the final hidden layer from each model--which is of a low dimension that the researcher controls--and match on the union of these two hidden objects.
			
			\item[2b.] \textit{SANN (Siamese Artificial Neural Network)}: We estimate two SANN models, one to learn to place units with similar outcomes nearby each other on a low-dimensional manifold, and one to learn to place units with similar treatment status nearby each other on a low-dimensional manifold. We then remove the final embedding layer from each model--which is of a low dimension that the researcher controls--and match on the union of these two objects.
			
		\end{itemize}

\end{itemize}

A constant feature of each procedure above is that we estimate two separate models--one whose objective function makes use of outcome data and one whose objective function makes use of treatment status. \textbf{As will be shown in Section \ref{sec:econometric_framework}, this grants us a double robustness property as we need only to have consistent selection (in the feature selection case) or learning (in the feature learning case) in one of these domains in order for downstream estimation of treatment effects to be consistent. XXX Do we still plan to attempt to show this in this paper? XXX}

%This is done with the aim of achieving some idea of \textit{double selection}, following Belloni, Chernozhukov, and Hansen (2013).
In Section \ref{sec:estimators}, we present a more formal description of the above estimators, as well as their connection to double selection.
